Annotation of Car Trajectories based on Driving Patterns

Nowadays, the ubiquity of various sensors enables the collection of voluminous datasets of car trajectories. Such datasets enable analysts to make sense of driving patterns and behaviors: in order to understand the behavior of drivers, one approach is to break a trajectory into its underlying patterns and then analyze that trajectory in terms of derived patterns. The process of trajectory segmentation is a function of various resources including a set of ground truth trajectories with their driving patterns. To the best of our knowledge, no such ground-truth dataset exists in the literature. In this paper, we describe a trajectory annotation framework and report our results to annotate a dataset of personal car trajectories. Our annotation methodology consists of a crowd-sourcing task followed by a precise process of aggregation. Our annotation process consists of two granularity levels, one to specify the annotation (segment border) and the other one to describe the type of the segment (e.g. speed-up, turn, merge, etc.). The output of our project, Dataset of Annotated Car Trajectories (DACT), is available online at https://figshare.com/articles/dact_dataset_of_annotated_car_trajectories/5005289 .

==> Robot.tex <==
\section{Simple Automated Annotation}
\label{sec:robot}
During initial investigations on the data received from annotators, we observed some obvious patterns in the way annotations are made. This motivated us to think of a procedural way to implement those patterns. We build an automated annotator called {\sc AutoAnn} whose logic is based on speed-based, position-based and heading-based heuristics. {\sc AutoAnn}'s heuristics originate from human-based annotations and detects both segment borders (annotations) and segment types. However, employed heuristics are very simplistic and cannot replace the human power of decision making. Nonetheless, the benefit of an automated annotator is two-folded.

\begin{itemize}[leftmargin=*]
    \item The automated annotator can take after simple human logic points. Hence it can replace the subjectivity in human decisions.
    \item Being provided alongside human annotations, it enables experts to get to a consensus among annotators.
\end{itemize}

In DACT, we exploit automated annotations as an additional source for annotating car trajectories. {\sc AutoAnn} scans each single point in a trajectory (in the ascending order of timestamps) and makes comparisons with $k$ neighbor points. The $k$ parameter depends on the temporal precision of records in the dataset. Based on our data observations, we experimentally set $k = 5$. Given the temporal precision of our dataset, i.e., seconds, $k=5$ implies that we analyze behaviors in a $5$-second time window. For a given point $p$ and its $k$ neighbor points, {\sc AutoAnn} preforms following heuristics.

\begin{itemize}[leftmargin=*]
    \item Speed-wise, if $p$ falls into a local maxima among it's $k$ neighbors (i.e., $k$ previous and $k$ subsequent points), then $p$ marks the end of a ``speed-up'' segment.
    \item Similarly, if $p$ falls into a local minima, $p$ marks the end of a ``slow-down'' segment.
    \item If $p$ holds as the end of a ``slowdown'' and the speed at $p$ is lower than a threshold, then $p$ marks the end of a ``traffic-jam'' segment. Based on our data observation, we experimentally set the low speed threshed to $9$ miles per hour. The intuition is that a {\em serious} slow-down should be due to a traffic jam. Normal slowdowns may occur due a slight turn or sun rays where the speed does not get lower than $9$ miles per hour.
    \item If the speed of all $k$ previous points of $p$ are lower than the low speed threshold and the speed of the immediate point after $p$ is larger then the low speed threshed, the $p$ marks the end of a ``traffic-light'' segment.
    \item We define {\em heading-change} as the first-order derivative of $p$'s and $p'$'s heading values where $p'$ is the immediate point after $p$. To simplify computation, we replace {\em derivatives} with the mathematical subtraction. The point $p$ marks the end of a ``turn'' segment iff it satisfies following conditions: $(i)$ The heading-change of $k$ neighbors of $p$ are zero and $(ii)$ The heading-change at $p$ is larger than a threshold. We experimentally set the high heading change threshold to $15$. 
    \item If the position of the point $p$ is merely identical with the point $p'$ which happened before $p$, then $p'$ marks the beginning and $p$ marks the end of a ``loop'' segment. The intuition is that when a driver performs a loop (for instance through a highway exit), the first and last locations of the loop are identical with a tiny error. However, this position-based heuristic cannot be applied on our data because the same situation is reported when the car is still. A part of our future work is to make this heuristic more sophisticated. One potential extension is to consider speed, the heuristic which seems to be valid is $p$'s speed is larger than a minimum threshold.
\end{itemize}

On our data, {\sc AutoAnn} generated 2418 segments among which 10\% are speed-ups, 59\% are slow-downs, 6\% are traffic-jams, 20\% are traffic-lights and 5\% are turns. Of course {\sc AutoAnn} introduces many false positives and false negatives. 
%A comparison with table XXX shows that YYY. 
Although more advanced and learning-based heuristics can be considered for automated annotation, the goal in the current version is to implement simplistic human patterns in order to obtain a standard rule for comparing human annotations.
